Hybrid hypercomputing: towards a unification of quantum and classical computation

We investigate the computational power and unified resource use of hybrid quantum-classical computations, such as teleportation and measurement-based computing. We introduce a physically causal and local graphical calculus for quantum information theory, which enables high-level intuitive reasoning about quantum information processes. The graphical calculus defines a local information flow in a computation which satisfies conditions for physical causality. We show how quantum and classical processing units can now be formally integrated, and give an analysis of the joint resources used in a typical measurement-based computation. Finally, we discuss how this picture may be used to give a high-level unified model for hybrid quantum computing.

==> coms.tex <==

\newcommand{\ket}[1]{\ensuremath{|#1 \rangle}}
\newcommand{\bra}[1]{\ensuremath{\langle #1|}}
\newcommand{\braket}[2]{\ensuremath{\langle #1|#2 \rangle}}
\newcommand{\ketbra}[2]{\ensuremath{|#1 \rangle \langle #2|}}
\newcommand{\ro}[1]{\ensuremath{|#1 \rangle \langle #1|}}
\newcommand{\av}[1]{\ensuremath{\langle #1 \rangle}}

\newcommand{\real}{\ensuremath{\mathrm{Re}}}
\newcommand{\trace}{\ensuremath{\textsf{Tr}}}

\newcommand{\id}{\ensuremath{\mathsf{1}}}
\newcommand{\iden}{\ensuremath{{\sf 1\hspace*{-1.0ex}\rule{0.15ex}
{1.2ex}\hspace*{1.0ex}}}}
\newcommand{\R}{\ensuremath{{\sf R\hspace*{-0.9ex}\rule{0.15ex}
{1.5ex}\hspace*{0.9ex}}}}
\newcommand{\N}{\ensuremath{{\sf N\hspace*{-1.0ex}\rule{0.15ex}
{1.3ex}\hspace*{1.0ex}}}}
\newcommand{\Q}{\ensuremath{{\sf Q\hspace*{-1.1ex}\rule{0.15ex}
{1.5ex}\hspace*{1.1ex}}}}
\newcommand{\C}{\ensuremath{{\sf C\hspace*{-0.9ex}\rule{0.15ex}
{1.3ex}\hspace*{0.9ex}}}}
%% for integers, do \usepackage{amssymb} in the preamble and
%% then $\mathbb{Z}$ for the symbol where required.


\newcommand{\h}[1]{\ensuremath{\mathcal{H}_{#1}}}

\newcommand{\me}{\ensuremath{\mathrm{e}}}
\newcommand{\mi}{\ensuremath{\mathrm{i}}}

\newcommand{\de}{\ensuremath{\mathrm{d}}}
\newcommand{\dd}[2]{\ensuremath{\frac{\mathrm{d}#1}{\mathrm{d}#2}}}
\newcommand{\ddd}[2]{\ensuremath{\frac{\mathrm{d}^2#1}{\mathrm{d}#2^2}}}

\newcommand{\ot}[2]{\ensuremath{\left( \begin{array}{c} #1 \\ #2
\end{array} \right)}}
\newcommand{\oth}[3]{\ensuremath{\left( \begin{array}{c} #1 \\ #2 \\ #3
\end{array} \right)}}
\newcommand{\twtw}[4]{\ensuremath{\left( \begin{array}{cc} #1 & #2 \\
#3 & #4 \end{array} \right)}}
\newcommand{\thth}[9]{\ensuremath{\left( \begin{array}{ccc} #1 & #2 & #3
\\ #4 & #5 & #6 \\ #7 & #8 & #9 \end{array} \right)}}


\newcommand{\expp}[1]{\ensuremath{\me^{\mi\hat{H}#1}}}
\newcommand{\expm}[1]{\ensuremath{\me^{-\mi\hat{H}#1}}}

\newcommand{\q}{\ensuremath{q_{ai}}}
